Revisiting Methods for Finding Influential Examples

Several instance-based explainability methods for finding influential training examples for test-time decisions have been proposed recently, including Influence Functions, TraceIn, Representer Point Selection, Grad-Dot, and Grad-Cos. Typically these methods are evaluated using LOO influence (Cook's distance) as a gold standard, or using various heuristics. In this paper, we show that all of the above methods are unstable, i.e., extremely sensitive to initialization, ordering of the training data, and batch size. We suggest that this is a natural consequence of how in the literature, the influence of examples is assumed to be independent of model state and other examples -- and argue it is not. We show that LOO influence and heuristics are, as a result, poor metrics to measure the quality of instance-based explanations, and instead propose to evaluate such explanations by their ability to detect poisoning attacks. Further, we provide a simple, yet effective baseline to improve all of the above methods and show how it leads to very significant improvements on downstream tasks.

==> Extras/extra.tex <==
\subsection{Leave One Out:}
\begin{center}

\begin{tabular}{ c c c c }
  \toprule
    \textbf{Pearson} & \textbf{Kendal} & \textbf{Spearman} & \textbf{Top 10 Matching} \\
    \midrule
    \multicolumn{4}{c}{Initialization} \\
    \midrule
    0.206 & 0.199 & 0.259 & 8.21 / 20.0 \\
    0.188 & 0.242 & 0.315 & 6.8 / 20.0 \\
    0.178 & 0.206 & 0.259 & 7.36 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{Ordering} \\
    \midrule
    0.159 & 0.14 & 0.2 & 4.31 / 20.0 \\
    0.149 & 0.091 & 0.133 & 3.47 / 20.0 \\
    0.186 & 0.109 & 0.152 & 4.14 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{batch Size} \\
    \midrule
    0.25 & 0.169 & 0.233 & 7.05 / 20.0 \\
    0.16 & 0.205 & 0.291 & 6.61 / 20.0 \\
    0.402 & 0.215 & 0.302 & 6.32 / 20.0 \\
  \bottomrule
\end{tabular}


\subsection{TraceInIdeal:}

\begin{tabular}{ c c c c }
  \toprule
    \textbf{Pearson} & \textbf{Kendal} & \textbf{Spearman} & \textbf{Top 10 Matching} \\
    \midrule
    \multicolumn{4}{c}{Initialization} \\
    \midrule
    0.7 & 0.538 & 0.683 & 14.33 / 20.0 \\
    0.776 & 0.704 & 0.834 & 17.27 / 20.0 \\
    0.739 & 0.644 & 0.764 & 14.06 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{Ordering} \\
    \midrule
    0.184 & 0.488 & 0.699 & 6.78 / 20.0 \\
    0.102 & 0.43 & 0.636 & 6.25 / 20.0 \\
    0.132 & 0.489 & 0.697 & 6.32 / 20.0 \\
    \midrule
  \bottomrule
\end{tabular}


\subsection{TraceinCP:}

\begin{tabular}{ c c c c }
  \toprule
    \textbf{Pearson} & \textbf{Kendal} & \textbf{Spearman} & \textbf{Top 10 Matching} \\
    \midrule
    \multicolumn{4}{c}{Initialization} \\
    \midrule
    0.781 & 0.406 & 0.566 & 9.38 / 20.0 \\
    0.848 & 0.602 & 0.76 & 12.08 / 20.0 \\
    0.718 & 0.536 & 0.706 & 10.41 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{Ordering} \\
    \midrule
    0.882 & 0.797 & 0.924 & 14.67 / 20.0 \\
    0.825 & 0.73 & 0.868 & 13.27 / 20.0 \\
    0.849 & 0.7 & 0.833 & 12.57 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{batch Size} \\
    \midrule
    0.833 & 0.629 & 0.797 & 11.27 / 20.0 \\
    0.435 & 0.546 & 0.735 & 10.07 / 20.0 \\
    0.628 & 0.762 & 0.925 & 14.0 / 20.0 \\
  \bottomrule
\end{tabular}

\section{RPS:}

\begin{tabular}{ c c c c }
  \toprule
    \textbf{Pearson} & \textbf{Kendal} & \textbf{Spearman} & \textbf{Top 10 Matching} \\
    \midrule
    \multicolumn{4}{c}{Initialization} \\
    \midrule
    0.868 & 0.616 & 0.827 & 9.92 / 20.0 \\
    0.86 & 0.803 & 0.936 & 14.7 / 20.0 \\
    0.787 & 0.693 & 0.886 & 10.92 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{Ordering} \\
    \midrule
    0.856 & 0.90 & 0.969 & 16.67 / 20.0 \\
    0.884 & 0.899 & 0.985 & 15.32 / 20.0 \\
    0.87 & 0.898 & 0.969 & 16.95 / 20.0 \\
    \midrule
    \multicolumn{4}{c}{batch Size} \\
    \midrule
    0.897 & 0.818 & 0.954 & 15.31 / 20.0 \\
    \midrule
  \bottomrule
\end{tabular}



\end{center}

\section{Why?}

\textbf{TraceIn: The state of NN is ignored} When the model moves from state $W_t$ to $W_{t+1}$ because of a sgd step on a single training example $x_i$, the change in loss on the test data $x_j$ is defined as the influence of $x_i$ on the test example $x_j$. This should have been Influence of $x_i$ on $x_j$ given the model state $W_t$. 

\begin{align*}
    Tracein: I(x_{train}, x_{test}) &= L(x_{test}| W_{t}) - L(x_{test} | W_{t+1}) \\
    Correct: I(x_{train}, x_{test}| W_t) &= L(x_{test}| W_{t}) - L(x_{test} | W_{t+1})
\end{align*}

Calculating the influence conditioned on the model is not very useful. 
\begin{itemize}
    \item For interpretability: we should say that "When the neural network was at the state $W_t$, the training data $X_{train}$ influenced the test data $x_{test}$". 
    \item Say that the model predicted wrong label for a test data  $x_{test}$, and we found that $X_{train}$ was the most influential training data. Removing $x_train$ may not be always useful.
\end{itemize}

One useful measure could be expected influence $E_{W_t}[I(x_{train}, x_{test}| W_t)]$. The Good part is, TraceIn does some kind of expectation (sums over a few $W_t$). 

Note that it is hard to find the unbiased expectation because we do not know how to properly sample $W_t$ (we do not know the distribution of $W_t$ -- The probability of seeing $W_t$ as a weight in training step).

\textbf{Leave One Out:} The issue is same with Leave one out as well. The current assumption is that the total reduction in loss is the sum of influence of all the training examples and therefore when we remove one training example and retrain the model the difference between the new and the old loss is the influence of the removed training example. However, this is wrong -- The total reduction in the loss is sum of influence of each training example conditioned on their respective model states. 


\textbf{Influence Functions: } Can we think of influence functions as some kind of expectations over the state? With the current formulation there is no issue of state (but the influence is with respect to the Global optima).


\section{RPS Possibly erroneous interpretation: } 

Let us analyse RPS for regression (MSE Loss), 

\begin{align*}
    I(x_i, x) &=  \alpha_i f_i^Tf \\
    \text{where } \alpha_i &= \frac{-1}{2\lambda n} \frac{\partial L(x_i, y_i, \Theta) }{\partial \Phi (x_i, \Theta) } \\
\end{align*}

For regression ($l_2$ loss), 

\begin{align*}
    L(x_i, y_i, \Theta) &= (\Phi (x_i, \Theta) - y_i)^2 \\
    \frac{\partial L(x_i, y_i, \Theta) }{\partial \Phi (x_i, \Theta) } &= 2(\Phi (x_i, \Theta) - y_i) \\
    I(x_i, x) &= \frac{-1}{\lambda n} \big[ \Phi (x_i, \Theta) - y_i)\big] f_i^Tf \\
\end{align*}

$ \Phi (x_i, \Theta) $ is the final prediction of the model. The above equation says if the model predicts an example perfectly, then the influence of that example is $0$, which is very counter intuitive. 

\textbf{Why traditional kernel methods (Gaussian Process regression) are interpretable?} 

The mean of predictive posterior of Gaussian process regression is given by 
\begin{align*}
    \mu (x_*) &= k_*^T C_N^{-1} y \\
    \text{where }  k_* &= [k(x_1, x_*) , ... k(x_i, x_*) ...]^T \\
    \text{and } C_N[i, j] &= k(x_i, x_j) + \sigma^2 I(i == j) 
\end{align*}

We can look the above equation in 2 ways 
\begin{align*}
    \text{interpretation 1: } \mu (x_*)  &= k_*^T \alpha \\
    &= \sum_{i=1}^{N} k(x_i, x_*) \alpha_i \\
    \text{interpretation 2: } \mu (x_*)  &= \beta  y \\
     &= \sum_{i=1}^{N} \beta_i  y_i
\end{align*}

interpretation 1 may not give us influence because  the $\alpha_i$ is not just a function of $i^{th}$ data point but depends on the entire dataset. RPS uses this interpretation and hence we may not get a very useful influence metric. 

However, the interpretation 2 is quite useful, the $\beta_i$ directly gives the influence of $i^{th}$ example, under the following definition of influence 

\textbf{Influence: } For the training point $x_i$ if we change $y_i$ to $y_i + \delta$ (not necessarily small) then what is the change in prediction 

Note that the $\beta_i$ term is independent of y's. Therefore, the change in prediction id $\beta_i * \delta$.

\subsection{What to do next:} 

Borrow the inspiration from RPS and use interpretation 2 instead of interpretation 1. 

\textbf{Approach 1:} 

In essence, RPS takes a trained neural network and approximates the final \textit{multivariate linear Regression} ($z \to \Phi(x) $) to a non parametric form. Since we know $(x_i, y_i) = (z_i, \Phi(x_i) $ for the multivariate regression we can use the above equation (predictive mean of Gaussian Process) to approximate to a non parametric form of interpretation 2. 

\textbf{Cons:}
\begin{itemize}
    \item $O(N^3)$ complexity. Although a lot of approximations are available for GP regression. 
    \item unlike GP regression, we don't directly get the influence which tells us what happens when we change $y_i$ to $y_i + \delta$. instead we get what happens when we change $\Phi(x_i) to \Phi(x_i) + \delta $. Nonetheless, for a well fitted model $\Phi(x_i)$ is similar to $y_i$ (after sigmoid). 
\end{itemize}

\textbf{Approach 2:} 

From the definition of the influence we defined before, we can think it as follows -- what happens to the prediction if we flip the label of the $i^{th}$ training data point. In other words, what happens to  prediction (or loss) if I down sample $(x_i, y_i)$ and up sample $(x_i, y_i^{error})$. This is simply the influence function applied twice (once to down sample and other to up sample with changed y). 



\textbf{Approach 3:} 

Can we approximate the final multivariate linear regression by any other interpretable model. 





\section{TraceIn: A different interpretation}

TraceIn approximation can be seen in multiple ways when we think from the above perspective (taking state into account). 

\begin{align}
    TraceInCP(x_{tr}, x_{ts}) &= \sum_{i=1}^{k}\eta \nabla l (W_{i}, x_{tr}) \nabla l (W_{i}, x_{ts}) \\
    &= \sum_{i=1}^{k} L(x_{ts}| W_i ) - L(x_{ts} |W_{i+1}(x_{tr}) ) 
\end{align}

\textbf{Interpretation 1:} If we define $I(x_{train}, x_{test}| W_t) = L(x_{test}| W_{t}) - L(x_{test} | W_{t+1})$ then the equation (2) can be seen as average over a fixed sample of $W$. The only difference between TraceInIdeal and TraceInCP is the way of sampling $W$

\textbf{Interpretation 2:} Since we are using gradient descent, the component of gradient of training point $x_{tr}$ at $W_t$ along the gradient of test point $x_{ts}$ can be thought of $I(x_{train}, x_{test}| W_t)$. (This requires some normalisation to the equation).

\subsection{Some other possible conditional influences:}

\begin{align}
    TraceInCP(x_{tr}, x_{ts}) &= \sum_{i=1}^{k} \frac{\nabla l (W_{i}, x_{tr}) \nabla l (W_{i}, x_{ts}) }{|\nabla l (W_{i}, x_{ts})|} \\
    TraceInCP(x_{tr}, x_{ts}) &= \sum_{i=1}^{k} Cos( \nabla l (W_{i}, x_{tr}), \nabla l (W_{i}, x_{ts}) )
\end{align}




==> Extras/introduction_old.tex <==

Local methods for finding influential examples such as {\em influence sketching} \cite{Wojnowicz_2016} and {\em influence functions} \cite{pmlr-v70-koh17a} are computationally expensive, and while fast heuristics have been proposed \cite{guo2020fastif}, the inference times associated with these methods are prohibitive of large-scale applications. In response, various global methods have been proposed that compute direct mappings of input examples into influence attributions, including {\em representer point selection} (RPS) \cite{yeh2018representer} and {\em TracIn} \cite{pruthi2020estimating}. Since these methods are a lot faster than their local counterparts, we would expect them to perform worse (be less {\em faithful} \cite{jacovi-goldberg-2020-towards}), but how do we feasibly evaluate instance-based explanation methods? \cite{hanawa2020evaluation} recently proposed a set of heuristics. This paper discusses several limitations of RPS and TracIn, as well as of these evaluation heuristics:

\begin{itemize}
    \item RPS influence estimates are sensitive to vector norms of training examples, which -- in the context of language modeling, for example -- arguably lead to a bias against vague examples. We highlight this with synthetic examples. 
    \item TracIn influence estimates are sensitive to random initializations, as well as batch sizes. We show this effect on both synthetic and real datasets. 
    \item The heuristics in \cite{hanawa2020evaluation} are trivially satisfied by some methods and almost never satisfied by others; for neural networks, they are sensitive to random initializations.
    \item We identify a source of confusion that we speculate motivated the heuristics in \cite{hanawa2020evaluation}: the distinction between influence and {\em usefulness}. We provide (synthetic) examples where useful data points, correctly identified by these heuristics, are not influential. 
\end{itemize}

We propose two ways of improving RSP and TracIn: 

\begin{itemize}
    \item RSP can be improved by a simple normalization trick. We call this RSP$^+$. 
    \item TracIn can be stabilized by simply averaging over random restarts. We call this TracIn$^+$.
    \item Inspired by recent work on supervised and unsupervised concept activation \cite{kim2018interpretability,ghorbani2019automatic}, we propose a novel heuristic for evaluating instance-based explainability methods. We see this heuristics leads to {\em both} detecting more useful data points {\em and} much higher agreement with leave-one-out influence (Cook's distance). 
    %\item We show that RSP$^+$ and TracIn$^+$ outperform their baselines, both in terms of our novel heuristic and in terms of leave-one-out influence.
\end{itemize}


==> Extras/limitations.tex <==
\begin{center}
\begin{table}





\begin{tabular}{c c c c | c c c   }
  \toprule
     & \multicolumn{3}{c|}{\textbf{MNIST}} & \multicolumn{3}{c}{\textbf{CoMNIST}} \\
      \midrule
    \textbf{Type} &  \textbf{Pearson} & \textbf{Spearman} & \textbf{Top 10\% Match} & \textbf{Pearson} & \textbf{Spearman} &  \textbf{Top 10\% Match} \\
    \midrule
    & \multicolumn{6}{c}{\textbf{Sensitivity to Initialization}} \\
    \midrule
     \textbf{Leave One Out} & 0.048  & 0.012  &  15.37 \% & 0.006 &  0.002 &  14.46\%\\ 
     \textbf{TraceIn Ideal} & 0.422 & 0.524 & 45.08\% & 0.442 &  0.666 &  50.11 \%\\ 
     \textbf{TraceIn CP} & 0.782 & 0.849 &  57.14\%  & 0.8 &  0.937 &  66.21\% \\
     \textbf{RPS} &  0.862 & 0.906 & 63.72\% & 0.628 &  0.897 &  63.77\% \\
    \midrule
    & \multicolumn{6}{c}{\textbf{Sensitivity to random ordering of training data}} \\
    \midrule
    \textbf{Leave One Out} & 0.121 & 0.039  &  12.95\% & 0.009 &  0.009 &  10.76\% \\
    \textbf{TraceIn Ideal} & 0.095 & 0.453 & 23.27\% & 0.212 &  0.523 &  30.28\%\\
    \textbf{TraceIn CP} & 0.836 & 0.957 &  79.27\% & 0.83 &  0.958 &  77.52\%\\
    \textbf{RPS} & 0.972 & 0.982 & 84.29\%  & 0.696 &  0.934 &  77.87\%\\
    \midrule
    & \multicolumn{6}{c}{\textbf{Sensitivity to batch size}} \\
    \midrule
    \textbf{Leave One Out} & 0.146 & 0.088 &  22.66\% & 0.02 &  0.024 &  15.26\%\\
    \textbf{TraceIn CP} & 0.722  & 0.964 &  78.26\% & 0.846 &  0.953 &  72.29\%\\ 
    \textbf{RPS} & 0.936 & 0.98  & 80.97\%  & 0.693 &  0.904 &  69.59\%\\ 
  \bottomrule
\end{tabular}
\caption{\label{tab:mnist_sensitivity}\textbf{Sensitivity of various influence metrics:} We change only the initialisation of the model and fix everything else; For 2 different initialisation, For each of the 200 test example, we calculate the influence score for each of the training examples and find the average correlation metrics (Pearson, Spearman, Kendall and top 10\% match) between the influence scores; correlations  averaged across the test examples. We repeat the above process for multiple pairs of initialisation. Similarly, we only change the random ordering of training data and only change the batch size, fixing everything else. }
\end{table}
\end{center}


\begin{itemize}
    \item Should we include influence functions, Grad-Dot, Tracein-Cos and Grad-Cos (which is same as Tracein-Cos but only the final CKPT is used)? should we include them in appendix? 
    \item 
\end{itemize}


\subsection{Influence Functions: }
\subsection{TracIn:}
\subsection{Leave-one-out: }
\subsection{Representer Point Selection: }




==> Extras/marginalized_influence.tex <==
\begin{center}
\begin{table}

\begin{tabular}{c c c c | c c c   }
  \toprule
     & \multicolumn{3}{c|}{\textbf{MNIST}} & \multicolumn{3}{c}{\textbf{CoMNIST}} \\
      \midrule
    \textbf{Type} &  \textbf{Pearson} & \textbf{Spearman} & \textbf{Top 10\% Match} & \textbf{Pearson} & \textbf{Spearman} &  \textbf{Top 10\% Match} \\
    \midrule
     \textbf{Leave One Out} & 0.575  &  0.111 & 14.83\% & 0.03  &  0.021 & 11.791\% \\ 
     \textbf{TraceIn Ideal} & 0.707  &  0.471 & 27.24\% & 0.699  &  0.853 & 63.861\% \\ 
     \textbf{TraceIn CP} & 0.937  &  0.942 & 76.06\% & 0.93  &  0.987 & 88.259\%  \\
     \textbf{RPS} & 0.995  &  0.995 & 93.285 & 0.943  &  0.927 & 87.215\% \\
  \bottomrule
\end{tabular}
\caption{\label{tab:marginal}\textbf{Sensitivity of marginalised influence metrics: } For each of the 200 test point, we can calculate the expected influence scores of each of the 1000 training example using two different disjoint sets of seeds and we report the correlation averaged over test examples.}
\end{table}
\end{center}


\subsection{Cross Correlation across methods:} 

\begin{center}
\begin{table}

\begin{tabular}{c c c c c }
  \toprule
  & \textbf{LeaveOneOut} & \textbf{TraceinIdeal} & \textbf{TraceinCP} & \textbf{RPS} \\
  \midrule
    \textbf{LeaveOneOut} & 1.0 & 0.113 & 0.124 & 0.122 \\
    \textbf{TraceinIdeal} & 0.113 & 1.0 & 0.655 & 0.654 \\
    \textbf{TraceinCP} & 0.124 & 0.655 & 1.0 & 0.944\\
    \textbf{RPS}  & 0.122 & 0.654 & 0.944 & 1.0\\
  \bottomrule
\end{tabular}
\caption{\label{tab:mnist_cross}\textbf{MNIST Correlation between various Influence metrics.} }
\end{table}
\end{center}


\begin{center}
\begin{table}

\begin{tabular}{c c c c c }
  \toprule
  & \textbf{LeaveOneOut} & \textbf{TraceinIdeal} & \textbf{TraceinCP} & \textbf{RPS} \\
  \midrule
    \textbf{LeaveOneOut} & 1.0 & -0.008 & -0.008 & -0.006 \\
    \textbf{TraceinIdeal} & -0.008 & 1.0 & 0.887 & 0.838 \\
    \textbf{TraceinCP} & -0.008 & 0.887 & 1.0 & 0.929\\
    \textbf{RPS}  & -0.006 & 0.838 & 0.929 & 1.0 \\
  \bottomrule
\end{tabular}
\caption{\label{tab:mnist_cross}\textbf{CoMNIST Correlation between various Influence metrics.} }
\end{table}
\end{center}







==> Extras/notes.tex <==

\section{Possible Heuristics/use cases (atleast in NLP):}

\begin{itemize}
    \item For a given cross lingual task, if a cross-lingual model predicts same class on an English sentence $S_{en}$ and its corresponding sentence in another language, $S_{lang}$ then the influential examples should be highly correlated. (If the model is predicting for the right reason).
    \item Local checklist invariance Test: Assume 2 data points $x_a$ and $x_b$ and we expect the model to be invariant for the both the data point (checklist invariance) then their influential examples should also be highly correlated. 
    \item Fairness: If the performance of model on across different demographic groups are same does it mean that the models decision are not based the demographic features? (not sure). If the model is actually fair, then 2 data points with demographic attribute as the only difference should have similar influential examples. 
\end{itemize}


==> Extras/poison_experiment.tex <==
\begin{center}
\begin{table}

\begin{tabular}{c c c c  }
  \toprule
  & \textbf{Poisoned data} & Clear (label = 0) & Clear (label = 1) \\
  \midrule
  \textbf{LeaveOneOut} & 1.5e-04  & -7.46e-05 & -8.14e-05\\
  \textbf{TraceinIdeal} & 0.585 & -0.136 & -0.0067 \\
  \textbf{TraceinCP} &  22.144 & -4.613 &  0.825 \\
  \textbf{RPS}  & 0.395 &   -0.215 &  0.0834 \\
  \bottomrule
\end{tabular}
\caption{\label{tab:mnist_cross}\textbf{MNIST Synthetic poisoned experiment}: 100 training examples of class zero are poisoned (added a trigger and converted to label 1) and the model is trained. All the test examples are poisoned. We expect that poisoned training examples to be much more influential and we observe the same.  }
\end{table}
\end{center}


\begin{center}
\begin{table}

\begin{tabular}{c c c c  }
  \toprule
  & \textbf{Poisoned data} & Clear (label = 0) & Clear (label = 1) \\
  \midrule
  \textbf{LeaveOneOut} &  7.96e-4  & 1.1e-03 &  3.58e-03 \\
  \textbf{TraceinIdeal} & 0.686 &  -0.493 &  0.1956 \\
  \textbf{TraceinCP} & 86.36 & -31.75 &  21.61 \\
  \textbf{RPS}  & 0.213 & -7.644 & 0.566 \\
  \bottomrule
\end{tabular}
\caption{\label{tab:mnist_cross}\textbf{CoMNIST Synthetic poisoned experiment}: 100 training examples of class zero are poisoned (added a trigger and converted to label 1) and the model is trained. All the test examples are poisoned. We expect that poisoned training examples to be much more influential and we observe the same.  }
\end{table}
\end{center}



==> section-tex-files/discussions.tex <==
\textcolor{red}{Only if space permits}
\begin{itemize}
    \item Expected RPS looks similar to TraceinCP -- is it true. 
    \item Influence function and Leave one out are much more stable on convex functions
    \item The intuition with RPS. 
\end{itemize}


